Optimal mini-batch and step sizes for SAGA

Recently it has been shown that the step sizes of a family of variance reduced gradient methods called the JacSketch methods depend on the expected smoothness constant. In particular, if this expected smoothness constant could be calculated a priori, then one could safely set much larger step sizes which would result in a much faster convergence rate. We fill in this gap, and provide simple closed form expressions for the expected smoothness constant and careful numerical experiments verifying these bounds. Using these bounds, and since the SAGA algorithm is part of this JacSketch family, we suggest a new standard practice for setting the step sizes and mini-batch size for SAGA that are competitive with a numerical grid search. Furthermore, we can now show that the total complexity of the SAGA algorithm decreases linearly in the mini-batch size up to a pre-defined value: the optimal mini-batch size. This is a rare result in the stochastic variance reduced literature, only previously shown for the Katyusha algorithm. Finally we conjecture that this is the case for many other stochastic variance reduced methods and that our bounds and analysis of the expected smoothness constant is key to extending these results.

==> sections/3_2_path.tex <==
%!TEX root = ../optimal_mini-batch.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Path to the optimal mini-batch size}
\label{sub:path_to_the_optimal_mini_batch_size}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Here, we aim to clarify our methodology.
The goal of this work is to find an optimal mini-batch size $b = |B|$ associated to the lowest total complexity denoted by $K_{\text{total}}$ (amount of computed stochastic gradients per iteration times the iteration complexity $K_{\mathrm{iter}}$) for a mini-batch SAGA algorithm with $b$-nice sampling.
In order to do so, we formulate our problem as the minimization of the total complexity
\begin{equation} \label{eq:init_pb}
  \text{find } b^* \in \argmin_{b = 1,\ldots,n} K_{\mathrm{total}}(b) \enspace.
\end{equation}
% After introducing the Lyapunov function used in convergence proofs of JacSketch $\Psi^k$
% \begin{equation*}
%   \Psi^k \eqdef \norm{w^k - w^*}_2^2 + \frac{\gamma}{2b L_{\max}} \norm{J^k - \nabla F(w^*)}_{\rm F}^2
% \end{equation*}
% where $\norm{\cdot}_{\rm F}$ denotes the Frobenius norm,
Theorems 3.6 and 4.19 of \citep{gower2018stochastic} imply that, in the case of mini-batch SAGA with $b$-nice sampling, the total
complexity\footnote{Note that $\lambda$ has been added to every smoothness constant since the analysis in~\citet{gower2018stochastic} depends on the $(L+\lambda)$-smoothness of $f$ and the $(L_B+\lambda)$-smoothness of the subsampled functions $f_B$.}
boils down to
\begin{equation} \label{eq:total_cplx_b_nice}
    \begin{aligned}[b]
        & K_{\mathrm{total}}(b) = b K_{\mathrm{iter}}(b)\\
        &\hspace{-5pt}= \max \hspace{-2pt} \Bigg\{ \Bigg. \hspace{-2pt} \frac{4b (\cL \hspace{-2pt} + \hspace{-2pt} \lambda)}{\mu}, n + \frac{n-b}{n-1}\frac{4(L_{\max} \hspace{-2pt} + \hspace{-2pt} \lambda)}{\mu} \hspace{-2pt} \Bigg. \Bigg\} \hspace{-2pt} \log\left( \frac{1}{\epsilon} \right),
    \end{aligned}
\end{equation}
with $\epsilon >0$ is the desired precision.

Unfortunately, computing $\cL$ turns out to be intractable when $n$ is large since we need to compute the mini-batch smoothness constant for all the possible mini-batches,
that is passing through all $b$-combinations from $n$.
This is why we look for upper bounds of $\cL$ leading us to upper bounds of the total complexity
\begin{equation*}
  K_{\mathrm{total}}(b) \leq \hat{K}_{\mathrm{total}} (b), \quad \forall b \in [n] \enspace.
\end{equation*}
Our aim is to find an argument of the minimum of this upper bound, that we hope is as tight as possible, denoted
\begin{equation} \label{eq:second_pb}
  \hat{b}^* \in \argmin_{b = 1,\ldots,n} \hat{K}_{\mathrm{total}}(b) \enspace,
\end{equation}
which is our estimation of the optimal mini-batch size.
This parameter $\hat{b}^*$ can be interpreted as the optimal mini-batch size in a pessimistic case, since we deduce it from an upper bound of the true complexity.

However, before producing any bound, one can easily compute exactly the expected smoothness constant for extreme cases.
If $b = 1$, one recovers the original SAGA algorithm with $\cL = \Lmax$
% \begin{align*}
%   \cL &= \frac{1 }{c_1} \max_{i=1,\ldots, n} \left\{\sum_{B \in \support(S) \,|\, i \in B } L_B \right\}\\
%   &= \max_{i=1,\ldots, n} L_i
%   = L_{\max} \enspace,
% \end{align*}
% where $c_1 = 1$ because $\cB$ reduces to the singletons of $[n]$.
because the possible batches are the singletons of $[n]$.
And if $b = n$, one recovers the traditional gradient descent algorithm for which the only possible batch is $[n]$, thus
%  $\cB = [n]$, $c_1 = 1$ and thus
$\cL = L$.
% \begin{align*}
%   \cL &= \frac{1}{c_1} \max_{i=1,\ldots, n} \left\{\sum_{B \in \support(S) \,|\, i \in B } L_B \right\}\\
%   &= \max_{i=1,\ldots, n} L_{[n]}
%   = L \enspace.
% \end{align*}
% So, this preliminary indication shows that our upper bounds should interpolate between $L_{\max}$ and $L$ respectively for $b = 1$ and $b = n$.


==> sections/4_1_larger_step_sizes.tex <==
%!TEX root = ../optimal_mini-batch.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Path to larger step sizes}
%\label{sub:path_to_larger_step_sizes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%First, we compare $1$-nice SAGA runs with a batch size of $b=1$, when $\cL = \cL_\text{practical} = \cL_\text{simple} = L_{\max}$, and different step sizes:
%\begin{itemize}
%    % \item $\gamma_{\text{Defazio}} = \frac{1}{3(n\mu + L_{\max})}$
%    % \item $\gamma_{\text{Hofmann}} = \frac{K}{2L_{\max}(1+K+\sqrt{1+K^2})}$ with $K\eqdef \frac{4L_{\max}}{n \mu}$
%    \item $\gamma_{\cL} (1) = \gamma_\text{practical} (1) = \gamma_\text{simple} (1) = \frac{1}{n\mu + 4L_{\max}}$
%    \item $\gamma_\text{Bernstein} (1) = \frac{1}{4L_{\max} + \max \left\{ \frac{16}{3}\log d L_{\max}, \; \mu n \right\}}$
%\end{itemize}
%
%a simple calculation $\left(4L_{\max} + n\mu \geq \sqrt{(4L_{\max})^2 + (n\mu)^2}\right)$ proves that $\gamma_{\text{Hofmann}} (1) \geq \gamma_{\text{practical}} (1)$, but in practice both are very close.
